Characterizing Deep Gaussian Processes via Nonlinear Recurrence Systems

Recent advances in Deep Gaussian Processes (DGPs) show the potential to have more expressive representation than that of traditional Gaussian Processes (GPs). However, there exists a pathology of deep Gaussian processes that their learning capacities reduce significantly when the number of layers increases. In this paper, we present a new analysis in DGPs by studying its corresponding nonlinear dynamic systems to explain the issue. Existing work reports the pathology for the squared exponential kernel function. We extend our investigation to four types of common stationary kernel functions. The recurrence relations between layers are analytically derived, providing a tighter bound and the rate of convergence of the dynamic systems. We demonstrate our finding with a number of experimental results.

==> 1-intro.tex <==

%%%% GENERAL BACKGROUND INFORMATION
Gaussian Process (GP) and Deep Neural Network (DNN) are two active research areas in machine learning community. Although they are different in model specifications and applications, there exist some close connections between GP and DNN in many aspects including model equivalence~\cite{Neal_thesis,jaehoon_1,matthews,jaehoon_2}. 

%%%%%% STATE OF THE FIELD
Inspired by DNNs, \acrfull{dgp}~\cite{deep_gp_2013} is a new promising class of models which are constructed by a hierarchical composition of Gaussian process. The strength of this model lies in its capacity to have richer representation power from the hierarchical construction and its robustness to overfitting from the probabilistic modeling.


%%%%%% PROBLEM/ RESEARCH QUESTION
However, there exists a pathology, stating that the increase in the number of layers degrades the learning power of~\acrshort{dgp}~\cite{pathology_deep_gp}. That is, the output of models becomes a constant-like function. It is important to develop theoretical understanding of this behavior, and therefore to have proper tactics in designing model architectures and parameter regularization for preventing such issue.

To explain such phenomena, we focus on studying a quantity which measures the difference of any two layer outputs, or in other words, the magnitude of each layer in~\dgp{}. 
Previous work~\cite{pathology_deep_gp} investigates the Jacobian matrix of a given model which can be analytically interpreted as the product of those in each layer. Because of the connection between the manifold of a function and the spectrum of its Jacobian, the authors show the degree of freedom is reduced significantly at deep layers. Another study~\cite{how_deep} examines the same quantity as ours, studying the ergodicity of the Markov chain to explain the pathology. In contrast to the existing literature, we present an approach that captures relations of our interest quantity between layers. The relations are recursively constructed between layers, taking into account GP hyperparameters so that the analysis can reflect the importance of these hyperparameters. Particularly, the recurrence relations give us a tight bound of the important quantity, and reveal the rate of convergence to fixed points. In fact, we can reason about the existence of pathology based on studying the fixed points of the recurrence relation. Under a systematic guideline, we can further extend our analysis for a number of popular kernels. Therefore, we are able to compare the qualitative difference among them which potentially becomes useful in the process of designing kernel functions. For example, the spectral mixture kernels are less likely to suffer the pathology. More importantly, in the light of the obtained recurrence relations, we recommend practical uses of our analysis for a~\dgp{} model. For instance, we can explain if a~\dgp{} model fails to learn from data.

This paper presents the following contributions: (1) we provide a new perspective of the pathology in~\dgp{} under the lens of chaotic methodology; (2) we show that the recurrence relation between layers gives us a sense of the rate of convergence to a fixed point; (3) we give a general instruction to form the recurrence relation for several kernel functions including the squared exponential kernel function, the cosine kernel function, the rational quadratic kernel function and the spectral mixture kernel; (4) we justify our findings with numerical experiment as well as demonstrating the applicability of recurrence relations in debugging~\dgps{} in practice.


==> 2-related-work.tex <==
% \textbf{Deep Gaussian Process and Bayesian neural network} 
The seminal work~\cite{mackay_bnn} was the first guideline on applying Bayesian approaches to learn neural networks.~\cite{Neal_thesis} pointed out the connection of Gaussian processes and random wide neural networks with one hidden layer. A method mimicking DNNs under recursive kernels can be found in~\cite{deep_kernel}.
It is noteworthy that there is a recent surge in developing GP-based theory to understand DNNs~\cite{jaehoon_1,matthews,jaehoon_2}. 


The issue in~\dgps{} was first described in~\cite{pathology_deep_gp}. The authors used the spectrum of Jacobian to reason about the capacity of deep networks. Beyond this observation, this work contains suggestions for fixing the pathology as well as various ways to construct deep models. 


A notable work~\cite{how_deep} presented a theoretical studying of~\dgps{}, considering a number of ways to construct models including composition between layers, constructing covariance function like in~\cite{Paciorek_2003}, and convolution of layers. Our paper stays within the scope of compositional construction for~\dgps{}.
Our findings share some similarity with this work~\cite{how_deep} about how to avoid the pathology in the squared exponential kernels. In contrast, our paper offers an in-depth view of the rate of convergence as well as a tight estimation that can use even for non-asymptotic situations. Such estimation, therefore, can apply to analyze~\dgps{} in practice. Moreover, we present an analysis for a number of common shift-invariant kernels.

Studying dynamics between layers can be found in the literature of DNNs~\cite{transient_chaos_dnn, deep_information_propagation}. The central idea of these work is to study recursive relations between layers that can capture interesting properties.

% \textbf{Inference in deep Gaussian process } 
Since the idea of deep Gaussian process was proposed in~\cite{deep_gp_2013}, there have been a series of attempts to extend and improve the inference for deep Gaussian process. Although learning~\dgps{} is challenging,~\cite{nested_deep_gp, auto_encode_deep_gp, expect_propagation_deep_gp, rff_deep_gp, doubly_deep_gp, hamiltonian_deep_gp, deep_gp_importance_weight} show some promising directions to make inference possible. Most of these approaches propose approximate inference algorithms to tackle the intractability of learning~\dgps{}.

==> 4-preliminary.tex <==
In this section, we will first revisit a classical result on computing the high-order moment of multivariate Gaussian. Then, we show how to obtain the moment in the bivariate case which will lead us to the findings in the next section.

\begin{thm}[Isserlis theorem~\cite{high_moment_gaussian}]
If $(X_1, X_2,\dots, X_n)$ is zero-mean multivarite Gaussian, then 
\begin{equation*}
    \expect[\prod_{i=1}^nX_i] = \sum_{p \in P^2_n}\prod_{(i,j) \in p} \Cov(X_i,X_j), 
\end{equation*}
where $P^2_n$ denotes all the partition of $n$ elements into 2-element subsets. $p \in P^2_n$ is a partition consisting of pairs $(i,j)$.
\label{thm:isserlis}
\end{thm}
This theorem says that the high-order moment of Gaussian random variables can be decomposed as the sum over all possible ways partitioning random variables into pairs and the product over pairs within a partition. The theorem plays an important role in physics research~\cite{isserlis_application, isserlis_application_3,isserlis_application_2}.

There are some highlight properties about this theorem: (1) If $n=2m + 1$, then $\expect[X_1 X_2 \dots X_{2m+1}] = 0$. If $n=2m$, the number of pair partitions is $(2m-1)!! = \frac{(2m)!}{2^mm!}$. Here $!!$ is the notation of double factorial. Note that counting the number partition as double factorial is related to the \emph{perfect matching} problem, shall be used in our proof of the next result. Readers may refer to~\cite{combinatorial} for further details.
\begin{prop}[High-order moment of bivariate Gaussian]
    Let (X,Y) be a multivariate zero-mean Gaussian vector. With $a, b \in \mathbb{N}$, $a+b=2c$, and $a \leq b$, the followings holds
    \begin{align*}
        \expect[X^aY^b] =& \sum_{i=1}^{\floor*{a/2}} \frac{a!b!}{2^{\frac{a - b + 4i}{2}} (a-2i)! i! (\frac{b - a + 2i}{2})!}\\
        %%%
        &\Cov(X,X)^{i}\Cov(X,Y)^{a-2i}\Cov(Y,Y)^{(b-a +2i) /2}.
    \end{align*}
    \label{prop:high_order_product}
\end{prop}
This result is a consequence of Isserlis theorem. It can can be viewed as Isserlis theorem with repetition in variables. In a simple example, the way to perform partitioning in Isserlis theorem can be understood as partitioning a set of ball with \emph{different} colors, while this proposition focuses on partitioning a set of balls with two colors \emph{red} and \emph{blue}, and keeps track of how many ways to have pairs such as (red, red), (red, blue), and (blue, blue). A detailed proof is in Appendix~\ref{appendix:high_order_product}.

==> 5.4-MARTERN.tex <==
\section{Mat\'ern kernel}
We only show our analysis on the most simplest form of Mat\'ern kernel as
\begin{equation}
    \textsc{MATERN}(\vx, \vx') = \sigma^2 \left(1 + \frac{\sqrt{3}r}{\ell}\right)\exp\left(-\frac{\sqrt{3}r}{\ell}\right),
    \label{eq:matern_kernel}
\end{equation}
where $r = \normx{\vx - \vx'}{2}$. However, this can be extended to the class function having half-integer value of $\nu=p + 1/2$.\\
\textbf{Finding recurrence} Analogous to the previous sections, we should come up with the expectation of 
\begin{align*}
     \expect[Z_l] =& 2m\sigma^2 - 2m\sigma^2\expect[\exp(-\frac{\sqrt{3}\sqrt{Z_{l-1}}}{\ell} )|\vf_{l-2}] + \\
     &2m\sigma^2\frac{\sqrt{3}}{\ell}\expect[\sqrt{Z_{l-1}}\exp(-\frac{\sqrt{3}\sqrt{Z_{l-1}}}{\ell})|\vf_{l-2}].
 \end{align*}
 Again, recall that $\frac{\sqrt{Z_{l-1}}}{\sqrt{s_{l-1}}}| \vf_{l-2} \sim \chi_m$. 
 The first expectation $\expect[\exp(-\frac{\sqrt{3}\sqrt{Z_{l-1}}}{\ell} )|\vf_{l-2}]$ can be obtained using the moment-generating function of Chi distribution. 
 
 The second expectation $\expect[\sqrt{Z_{l-1}}\exp(-\frac{\sqrt{3}\sqrt{Z_{l-1}}}{\ell})|\vf_{l-2}]$ is more tricky to obtain. To do so, we use  the following result:
 
 If $X \sim \chi_m$, for $k \geq 1$, then 
 \begin{equation}
     \expect[X^k \exp(tX)] = \sqrt{2^k}\frac{\Gamma((m+k)/2)}{\Gamma(m/2)} M_{\chi_{m+k}}(t).
 \end{equation}
 
Not only does this result allow us to study the Mat\'ern kernel in Equation~\ref{eq:matern_kernel} but also those of $\nu = p + \frac{1}{2}, p \geq 2$. The recurrence relation function for this kernel is rather complicated, and is a composition of multiple hypergeometric functions ${}_1F_1$. 

==> figure/graphical_models.tex <==
\begin{tikzpicture}
	\node[circle,draw=black,inner sep=0pt,minimum size=18pt,label=below:{$x$}] (a) at (0,0) {};
	
	\node[circle,draw=black,inner sep=0pt,minimum size=18,label=below:{$f_1(x)$}] (b) at (1.5,0) {};
	
	\node[circle,draw=black,inner sep=0pt,minimum size=18pt,label=below:{$f_2(x)$}] (c) at (3,0) {};
	
	\node[circle,draw=black,inner sep=0pt,minimum size=18pt,label=below:{$f_3(x)$}] (d) at (4.5,0) {};
	
	\draw[-> ] (a) edge (b);
	\draw[-> ] (b) edge (c);
	\draw[-> ] (c) edge (d);
	\draw[-> ] (a) edge[bend left] (c); 
	\draw[-> ] (b) edge[bend left] (d); 
\end{tikzpicture}
